Multi-Facet Blending for Faceted Query-by-Example Retrieval

With the growing demand to fit fine-grained user intents, faceted query-by-example (QBE), which retrieves similar documents conditioned on specific facets, has gained recent attention. However, prior approaches mainly depend on document-level comparisons using basic indicators like citations due to the lack of facet-level relevance datasets; yet, this limits their use to citation-based domains and fails to capture the intricacies of facet constraints. In this paper, we propose a multi-facet blending (FaBle) augmentation method, which exploits modularity by decomposing and recomposing to explicitly synthesize facet-specific training sets. We automatically decompose documents into facet units and generate (ir)relevant pairs by leveraging LLMs' intrinsic distinguishing capabilities; then, dynamically recomposing the units leads to facet-wise relevance-informed document pairs. Our modularization eliminates the need for pre-defined facet knowledge or labels. Further, to prove the FaBle's efficacy in a new domain beyond citation-based scientific paper retrieval, we release a benchmark dataset for educational exam item QBE. FaBle augmentation on 1K documents remarkably assists training in obtaining facet conditional embeddings.

==> content/finetune.tex <==
\section{Fine-tuning for QBE}

==> fig/tab_abla_temp.tex <==
\begin{table*}[t]
\centering
\scalebox{0.83}{
\begin{tabular}{lcccccccc}
\hline
CFSCUBE Facets  & \multicolumn{2}{c}{Background} & \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{Result} & \multicolumn{2}{c}{Aggregated} \\ \cline{2-9} 
Model  & NDCG$_{\%20}$ & MAP & NDCG$_{\%20}$ & MAP & NDCG$_{\%20}$ & MAP & NDCG$_{\%20}$ & MAP \\ \hline
SPECTER-COCITE$_{\texttt{Spec}}$ & 70.03 & \textbf{49.99}   & 45.99 & 25.60  & 59.95 & 37.33  & 58.38 & 37.39 \\
+MaBle$_{\texttt{Spec}}$      & \textbf{70.09} & 45.93 & \textbf{49.14} & \textbf{30.90} & \textbf{60.88} & \textbf{38.08} & \textbf{59.79} & \textbf{38.11}  \\ 
+MaBle-RN$_{\texttt{Spec}}$    & 69.61 & 46.58 & 46.82 & 28.62 & 59.83 & 37.47 & 58.48 & 37.32 \\
\hline
\end{tabular}}
\caption{Evaluation results of ablation study. While \textit{MaBle} includes the generation of \textit{dissimilar} aspects in Stage 2, \textit{MaBle-RN} selects \textbf{R}andom aspects as \textbf{N}egatives, and these aspects are chosen among the original aspects (decomposed summaries obtained in Stage 1) of the entire document set. \textit{+MaBle$_{\texttt{Spec}}$} and \textit{+MaBle-RN$_{\texttt{Spec}}$} denote fine-tuning on the above \textit{SPECTER-COCITE$_{\texttt{Spec}}$} with each method.}\label{table 3}
\end{table*}


==> fig/tab_hyperparameter.tex <==
\begin{table}[]
\centering
\scalebox{0.78}{%
\begin{tabular}{l|cc}
\hline
    & Hyperparameter & value  \\ \hline
Computing Infrastructure 
batch size & 0.756     & 0.668  \\
Sim & 0.736     & 0.634  \\ \hline
\end{tabular}%
} \caption{Averaged similarity scores between the whole document and each facet. \textit{Sum}: decomposed summary in Stage 1; \textit{Sim}: generated similar facets in Stage 2.}\label{tab: hyperparameter}
\end{table}
